Cell-Probe Lower Bounds and Complexity-Preserving Reductions for Suffix Array Queries

For a text $T$ of length $n$ over an alphabet of size $\sigma$, its suffix array lists the starting positions of the suffixes of $T$ in lexicographic order, and its inverse suffix array gives the lexicographic rank of the suffix starting at each position. Since the introduction of the FM-index and the compressed suffix array in 2000, both queries have been supported in $O((\log_\sigma n)^\epsilon)$ time using $O(n\log\sigma)$ bits, for any constant $\epsilon>0$. Yet no nontrivial time-space lower bound for suffix-array queries in compact space was known. We give the first such lower bound: in the cell-probe model with $\Theta(\log n)$-bit words, every deterministic $S$-bit data structure with $S\ge n$ answering suffix-array queries on binary strings of length at most $n$ has worst-case query time $\Omega(\log\log n/\log((S/n)\log\log n))$. Hence, structures with $O(n(\log\log n)^{O(1)})$ bits need $\Omega(\log\log n/\log\log\log n)$ query time, while constant query time requires $\Omega(n\log^\epsilon n)$ bits for some constant $\epsilon>0$, matching known upper bounds. In particular, no such $O(n)$-bit structure supports constant-time queries, answering the 25-year-old question of Grossi and Vitter. We also give exact complexity-preserving equivalences between suffix-array access and simpler prefix queries on short strings. For every $2\leq\sigma\leq n$, suffix-array queries are equivalent to prefix-select queries, and inverse-suffix-array queries are equivalent to prefix-special-rank queries. The reductions in both directions preserve all four standard measures up to constant factors: space, query time, preprocessing time, and preprocessing space. Unlike previous reductions, they incur no additive $O(\log\log n)$ query-time term. Thus, the corresponding prefix-query problems capture suffix-array and inverse-suffix-array access without asymptotic loss in any of the four measures.

==> settings.tex <==

%
\makeatletter
\newcommand{\refcheckize}[1]{%
  \expandafter\let\csname @@\string#1\endcsname#1%
  \expandafter\DeclareRobustCommand\csname relax\string#1\endcsname[1]{%
    \csname @@\string#1\endcsname{##1}\@for\@temp:=##1\do{\wrtusdrf{\@temp}\wrtusdrf{{\@temp}}}}%
  \expandafter\let\expandafter#1\csname relax\string#1\endcsname
}
\newcommand{\refcheckizetwo}[1]{%
  \expandafter\let\csname @@\string#1\endcsname#1%
  \expandafter\DeclareRobustCommand\csname relax\string#1\endcsname[2]{%
    \csname @@\string#1\endcsname{##1}{##2}\wrtusdrf{##1}\wrtusdrf{{##1}}\wrtusdrf{##2}\wrtusdrf{{##2}}}%
  \expandafter\let\expandafter#1\csname relax\string#1\endcsname
}
\makeatother

\refcheckize{\cref}
\refcheckize{\Cref}
\refcheckizetwo{\crefrange}
\refcheckizetwo{\Crefrange}

%
\makeatletter
\renewcommand\thmt@autorefsetup{\@xa\def\csname\thmt@envname autorefname\@xa\endcsname\@xa{\thmt@thmname}}
\makeatother

%
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{observation}[theorem]{Observation}
\crefname{observation}{Observation}{Observations}
\newtheorem{proposition}[theorem]{Proposition}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{construction}[theorem]{Construction}
\crefname{construction}{Construction}{Constructions}
\crefname{claim}{Claim}{Claims}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{example}[theorem]{Example}

%
%
\makeatletter
\AddToHook{env/theorem/before}{\if@nobreak\else\Needspace{2\baselineskip}\fi}
\AddToHook{env/definition/before}{\if@nobreak\else\Needspace{2\baselineskip}\fi}
\makeatother
\AddToHook{env/theorem/begin}{\crefalias{section}{theorem}}
\AddToHook{env/corollary/begin}{\crefalias{theorem}{corollary}}
\AddToHook{env/lemma/begin}{\crefalias{theorem}{lemma}}
\AddToHook{env/fact/begin}{\crefalias{theorem}{fact}}
\AddToHook{env/observation/begin}{\crefalias{theorem}{observation}}
\AddToHook{env/proposition/begin}{\crefalias{theorem}{proposition}}
\AddToHook{env/definition/begin}{\crefalias{theorem}{definition}}
\AddToHook{env/claim/begin}{\crefalias{theorem}{claim}}
\AddToHook{env/construction/begin}{\crefalias{theorem}{construction}}
\AddToHook{env/remark/begin}{\crefalias{theorem}{remark}}
\AddToHook{env/example/begin}{\crefalias{theorem}{example}}

%
%
%
\makeatletter
\let\paper@cref@resetby\cref@resetby
\renewcommand*\cref@resetby[2]{%
  \@ifundefined{alias@ctr@#1}{%
    \paper@cref@resetby{#1}{#2}%
  }{%
    \edef\paper@cref@next{%
      \noexpand\cref@resetby{\csname alias@ctr@#1\endcsname}}%
    \paper@cref@next{#2}%
  }%
}
\makeatother

%
%
\renewcommand{\theHtheorem}{\theHsection.\arabic{theorem}}

%
%
%
%
%
\makeatletter
\@ifundefined{if@skiphyperref}
  {\PackageError{paper}{Hyperref target suppression is unavailable}{}}
  {}
\newcommand{\paper@refstepcounterwithouttarget}[2]{%
  \let\paper@saved@skiphyperref\if@skiphyperref
  \@skiphyperreftrue
  #2%
  \let\if@skiphyperref\paper@saved@skiphyperref
  \hyper@makecurrent{#1}%
}
\newcommand{\thm@deferanchor}[2]{%
  \paper@refstepcounterwithouttarget{#1}{#2}%
  \edef\thm@anchor{%
    \noexpand\Hy@raisedlink{%
      \noexpand\hyper@anchorstart{\@currentHref}\noexpand\hyper@anchorend}}%
}
\let\thm@anchor\@empty
\patchcmd{\cref@thmnoarg}
  {\refstepcounter{#2}}
  {\thm@deferanchor{#2}{\refstepcounter{#2}}}
  {}{\PackageError{paper}{Cannot patch theorem destinations}{}}
\patchcmd{\cref@thmoptarg}
  {\refstepcounter[#1]{#3}}
  {\thm@deferanchor{#3}{\refstepcounter[#1]{#3}}}
  {}{\PackageError{paper}{Cannot patch shared-counter theorem destinations}{}}
\let\thm@original@deferredhead\deferred@thm@head
\def\deferred@thm@head#1{%
  \thm@original@deferredhead{\thm@anchor#1}%
  \let\thm@anchor\@empty
}
%
%
\@ifundefined{ttl@Hy@refstepcounter}
  {\PackageError{paper}{Cannot defer section destinations}{}}
  {\renewcommand{\ttl@Hy@refstepcounter}[1]{%
    \paper@refstepcounterwithouttarget{#1}{\refstepcounter{#1}}%
    \edef\ttl@Hy@saveanchor{%
      \noexpand\Hy@raisedlink{%
        \noexpand\hyper@anchorstart{\@currentHref}\noexpand\hyper@anchorend}}%
  }}
\makeatother

%
\newcommand{\creflastconjunction}{, and\nobreakspace}
\crefname{observation}{Observation}{Observations}
\Crefname{observation}{Observation}{Observations}

%
\definecolor{mypink}{RGB}{199, 21, 133}
\hypersetup{
  colorlinks,
  urlcolor = blue,
  linkcolor = mypink,
  citecolor = blue
}

%
\newcommand{\myparagraph}[1]{%
  \par\addvspace{3.25ex plus 1ex minus .2ex}%
  \noindent\textbf{#1}\quad\ignorespaces
}

%
%
%
%
%
%
%
%
%

%
%
%
%
%
%
%
%
%
%

%
\setul{2pt}{0.6pt}

%
\setlength{\FrameSep}{1.5ex}

%
\setlength{\OuterFrameSep}{\topsep}
\renewenvironment{framed}
  {\par\addvspace{\OuterFrameSep}%
   \ifdefined\nolinenumbers\nolinenumbers\fi
   \noindent\begin{minipage}{\linewidth}%
   \MakeFramed{\advance\hsize-\width\FrameRestore}}
  {\endMakeFramed\end{minipage}\par\addvspace{\OuterFrameSep}}

%
\setlist[enumerate]{nosep, topsep=1ex}
\setlist[itemize]{nosep, topsep=1ex}
\setlist[description]{nosep,topsep=1ex}

%
\allowdisplaybreaks

%
\lineskiplimit=-5pt

%
\let\oldabstract\abstract
\let\oldendabstract\endabstract
\makeatletter
\renewenvironment{abstract}
{\renewenvironment{quotation}%
  {\list{}{\addtolength{\leftmargin}{1.0em}%
    \listparindent 1.5em%
     \itemindent    \listparindent%
     \rightmargin   \leftmargin%
     \parsep        \z@ \@plus\p@}%
     \item\relax}%
  {\endlist}%
\oldabstract}
{\oldendabstract}
\makeatother

%
\fxsetup{mode=multiuser,theme=color, layout=inline}
\FXRegisterAuthor{tk}{atk}{\color{red} {\bf Tomasz}}
\FXRegisterAuthor{dk}{adk}{\color{green!70!black} {\bf Dominik}}

%
%
%
%
%
%
%
%
%
%
%

%
%
%
%
%
%

%
\newcommand{\DSComponents}{%
  \vspace{2ex}%
  \noindent%
  \textbf{\textit{Data structure}}\quad%
}
\newcommand{\DSQueries}{%
  \vspace{2ex}%
  \noindent%
  \textbf{\textit{Queries}}\quad%
}
\newcommand{\DSConstruction}{%
  \vspace{2ex}%
  \noindent%
  \textbf{\textit{Construction}}\quad%
}

%
\newenvironment{bfdescription}
  {\begin{description}[style=sameline,itemsep=0ex,font={\normalfont\bf}]}
  {\end{description}\vspace{-1.2ex}}

%
\renewcommand*\descriptionlabel[1]{\hspace\labelsep\normalfont\itshape #1}




